The Path to Proton Structure at One-Percent Accuracy

We present a new set of parton distribution functions (PDFs) based on a fully global dataset and machine learning techniques: NNPDF4.0. We expand the NNPDF3.1 determination with 44 new datasets, mostly from the LHC. We derive a novel methodology through hyperparameter optimisation, leading to an efficient fitting algorithm built upon stochastic gradient descent. We use NNLO QCD calculations and account for NLO electroweak corrections and nuclear uncertainties. Theoretical improvements in the PDF description include a systematic implementation of positivity constraints and integrability of sum rules. We validate our methodology by means of closure tests and "future tests" (i.e. tests of backward and forward data compatibility), and assess its stability, specifically upon changes of PDF parametrization basis. We study the internal compatibility of our dataset, and investigate the dependence of results both upon the choice of input dataset and of fitting methodology. We perform a first study of the phenomenological implications of NNPDF4.0 on representative LHC processes. The software framework used to produce NNPDF4.0 is made available as an open-source package together with documentation and examples.

==> tables/closure-outofsample-ratio.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\footnotesize
   \renewcommand{\arraystretch}{1.30}
\begin{tabular}{lrrr}
\toprule
{} & $\qquad$$n_{\rm dat}$ &  $\qquad$$\biasvarratio$ & $\qquad$ bootstrap error \\
Dataset &             &                  \\
\midrule
SeaQuest   &      &     0.99 &             0.10 \\
ATLAS      &      &    1.08 &             0.04 \\
CMS        &      &    1.04 &             0.05 \\
LHCb       &      &     0.92 &             0.07 \\
Total      &      &     1.03 &             0.05 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\caption{
  The bias-to-variance ratio
  $\biasvarratio$, defined in Eq.~(\ref{eq:BiasVarRatio_sqr}),
  divided by groups of processes and evaluated for the testing datasets
  that were not used as input to the NNPDF4.0 closure test fits.
  %
  The last column indicates the uncertainty associated to
  $\biasvarratio$,
  determined as its standard deviation 
over a bootstrap sample of both fits and replicas.
%
 Note that the combination of the training set used to evaluate Table~\ref{tab:delta-chi2-fitted}
 and the testing set shown here add up to the complete NNPDF4.0 baseline dataset.
 %
 For the total testing set, $\biasvarratio\simeq 1$ within this bootstrap error,
 demonstrating the faithfulness
 of the estimated PDF uncertainties.
}
\label{table:outofsample-ratio-closure}	
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/closure-outofsample-xi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.30}
 \begin{tabular}{lrrrr}
\toprule
{} &   $\xi^{(\rm data)}_{1\sigma}$ &  bootstrap error &  $\erf(\biasvarratio/\sqrt{2})$ &  bootstrap error \\
experiment &      &        &                 &        \\
\midrule
SeaQuest   & 0.67 &   0.05 &            0.69 &   0.05 \\
ATLAS      & 0.69 &   0.02 &            0.64 &   0.02 \\
CMS        & 0.67 &   0.03 &            0.67 &   0.02 \\
LHCb       & 0.68 &   0.04 &            0.72 &   0.03 \\
Total      & 0.68 &   0.02 &            0.67 &   0.03 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\caption{
  The one-sigma quantile estimator in the space of experimental
  data, $\xi^{(\rm data)}_{1\sigma}$, defined
  in  Eq.~(\ref{eq:XiDataDef}) and evaluated for the same
  testing dataset as that used for Table~\ref{table:outofsample-ratio-closure},
  together with the corresponding bootstrap error.
  %
  For each group of processes, we also display the value
  of  $\erf(\biasvarratio/\sqrt{2})$ evaluated using
  the corresponding bias-to-variance ratio.
  %
  As indicated by Eq.~(\ref{eq:expectedxi}), for
  a successful closure test one expects that 
  $\xi^{(\rm data)}_{1\sigma}\simeq \erf(\biasvarratio/\sqrt{2})$.
}
\label{table:outofsample-xi-closure}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/dataset-futuretest.tex <==
%-------------------------------------------------------------------------------
\begin{table}[t]
 \centering
 \footnotesize
 \renewcommand{\arraystretch}{1.30}
 \begin{tabular}{l|l|C{1.5cm}|C{1.5cm}|C{2.2cm}|C{1.6cm}}
   Process  &
   Dataset & pre-HERA  & pre-LHC  & NNPDF3.1-like & NNPDF4.0 \\
 \toprule
 \multirow{3}{*}{Fixed target DIS (NC)} &  BCDMS &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
 &  NMC &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
 &  SLAC &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
 \midrule
 \multirow{2}{*}{Fixed target DIS (CC)} &  CHORUS &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
 &  NuTeV &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
  \midrule
  \multirow{2}{*}{Fixed-target DY} &  E605 &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
 &  E866 &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark\\
 \midrule
 \multirow{3}{*}{HERA} &  HERA inclusive &    & \checkmark  &  \checkmark  &  \checkmark\\
 &  HERA charm &   & \checkmark  &  \checkmark  &  \checkmark\\
 &  HERA bottom &    & \checkmark  &  \checkmark  &  \checkmark\\
 \midrule
 \multirow{7}{*}{Collider DY (incl)} & CDF $Z$  &    &  \checkmark &  \checkmark  &  \checkmark\\
 & D0 $W,Z$  &    &  \checkmark &  \checkmark  &  \checkmark\\
 & ATLAS $W,Z$ 2010  &    &   &  \checkmark  &  \checkmark\\
 & CMS DY2D 2011  &    &   &  \checkmark  &  \checkmark\\
 & LHCb 7 TeV  &    &   &  \checkmark  &  \checkmark\\
 & LHCb 8 TeV  &    &   &  \checkmark  &  \checkmark\\
 & LHCb 13 TeV  &    &   &    &  \checkmark\\
 \midrule
 \multirow{2}{*}{Collider DY (w rad)} & ATLAS $Z$ $p_T$ 8 TeV  &    &   &  \checkmark  &  \checkmark\\
 & CMS $Z$ $p_T$ 8 TeV &    &   &  \checkmark  &  \checkmark\\
 \midrule
 \multirow{3}{*}{Top quark production} & ATLAS $t\bar{t}$ 8 TeV $l$+jets  &    &   &  \checkmark  &  \checkmark\\
 & CMS $t\bar{t}$ 8 TeV $l$+jets &    &   &  \checkmark  &  \checkmark\\
 & CMS single-top &    &   &    &  \checkmark\\
 \midrule
 \multirow{4}{*}{Jet data} & ATLAS 7 TeV dijets  &    &   &    &  \checkmark\\ 
  & CMS 7 TeV dijets  &    &   &    &  \checkmark\\
 & ATLAS 8 TeV incl. jets  &    &   &    &  \checkmark\\
 & CMS 8 TeV incl. jets  &    &   &    &  \checkmark\\
  \bottomrule
 \end{tabular}
 \vspace{0.3cm}
 \caption{\small The datasets that enter in each of the fits used for future testing, see text
 for details.
 %
 Each dataset is associated to a corresponding family of processes.
 %
 The collider Drell-Yan data are separated into inclusive measurements and
 measurements accompanied by extra radiation.
}
\label{table:dataset-futuretest}	
\end{table}
%-------------------------------------------------------------------------------


==> tables/delta_chi2_fitted.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
  \footnotesize
   \renewcommand{\arraystretch}{1.30}
\begin{tabular}{lrr}
\toprule
{} & $\qquad$ $\ndata$ &  $\qquad$ $\eshift{\Delta_{\chi^2}}$ \\
Dataset &        &                    \\
\midrule
DEUTERON   &    784 &          -0.0101 \\
NMC        &    204 &          -0.0030 \\
NUCLEAR    &    993 &          -0.0111 \\
HERACOMB   &   1208 &          -0.0054 \\
DYE886     &     89 &          -0.0273 \\
CDF        &     29 &          -0.0099 \\
D0         &     48 &          -0.0223 \\
ATLAS      &    326 &          -0.0057 \\
CMS        &    327 &          -0.0088 \\
LHCb       &     85 &          -0.0113 \\
Total      &   4093 &          -0.0087 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\small
  The expectation value of $\Delta_{\chi^2}$,
Eq.~(\ref{eq:deltachi2_def}), evaluated over the $n_{\rm fit}$ fits
that constitute the NNPDF4.0 closure test.
%
Results are presented separated into groups of datasets.
%
Recall that the data input to the closure tests is that of the NNPDF3.1-like dataset,
as discussed in the text.
%
One finds that  
$\eshift{\Delta_{\chi^2}} < 0$ for all datasets considered, indicating the absence of
under-fitting, while
its small absolute magnitude is consistent with proper learning. 
}
\label{tab:delta-chi2-fitted}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/table_dataset_variations.tex <==
%-------------------------------------------------------------------------------
\begin{table}[t]
 \centering
 \scriptsize
 \renewcommand{\arraystretch}{1.30}
 \begin{tabular}{|l|l|C{1.5cm}|C{1.5cm}|}
   Process  &
   Dataset & Global  & 3.1-like \\
   \toprule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{Fixed Target DIS}   & SLAC $p$, $d$  & \checkmark & \checkmark \\
   &  NMC $p$, $d/p$  & \checkmark& \checkmark\\
&  BCDMS $p$, $d$  & \checkmark& \checkmark\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     &  HERA I+II inclusive NC e+p 460 GeV  &     \\
  &  HERA I+II inclusive NC $e^+ + p$ 575 GeV  &     \\
  &  HERA I+II inclusive CC $e^- + p$  &     \\
  &  HERA I+II inclusive NC $e^- + p$  &     \\
  & NuTeV dimuon    &     \\
  &   ATLAS $\sigma_{tt}^{\rm tot}$  &     \\
&  LHCb $Z\to ee$ 2 fb    &     \\
  &  HERA comb. $\sigma_{c\bar c}^{\rm red}$  &     \\
  &  DY E886 $\sigma^p_{\rm DY}$  &     \\
  &  CMS W asymmetry 840 pb  &     \\
  &  CMS $t\bar{t}$ rapidity $y_{t\bar{t}}$  &     \\
  &  CHORUS   &     \\
  &  CMS W rapidity 8 TeV  &     \\
  &  ATLAS $t\bar{t}$ $y_t$  &     \\
  &  LHCb $W,Z \to \mu$ 7 TeV  &     \\
  &  ATLAS low-mass DY 2011  &     \\
  &  ATLAS Z pT 8 TeV $(p_T^{ll}, M_{ll})$  &     \\
  &  HERA I+II inclusive CC $e^+ + p$  &     \\
  &  D0 Z rapidity  &     \\
  &  CMS Drell-Yan 2D 7 TeV 2011  &     \\
  &  DY E605 $\sigma^p_{\rm DY}$  &     \\
  &  LHCb  $W,Z \to \mu$ 8 TeV  &     \\
  &  HERA comb. $\sigma_{b\bar b}^{\rm red}$  &     \\
  &  ATLAS $W,Z$ 7 TeV 2011 Central selection  &     \\
  &  CMS W asymmetry 4.7 fb  &     \\
  &  NMC p  &     \\
  &  DYE 866 $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$  &     \\
  &  ATLAS Z pT 8 TeV  $(p_T^{ll}, y_{ll})$  &     \\
  &  CDF Z rapidity  &     \\
  &  SLAC p  &     \\
  &  ATLAS HM DY 7 TeV  &     \\
  &  D0 $W\to \mu \nu$ asymmetry  &     \\
  &  CMS $\sigma_{tt}^{\rm tot}$  &     \\
  &  NuTeV    &     \\
  &  CMS Z pT 8 TeV $(p_T^{ll}, y_{ll})$  &     \\
  &  LHCb Z 940 pb  &     \\
  &  HERA I+II inclusive NC $e^+ + p$ 820 GeV  &     \\
  &  HERA I+II inclusive NC $e^+ + p$ 920 GeV  &     \\
  &  ATLAS $W, Z$ 7 TeV 2010  &     \\
  &  CHORUS   &     \\
  &  D0 $W\to e \nu$  asymmetry  &     \\
  &  CMS jets 7 TeV 2011  &     \\
  &  ATLAS jets 2011 7 TeV  &     \\
  &  ATLAS direct photon production 13 TeV  &     \\
  &  ATLAS single top Rt 7 TeV  &     \\
  &  ATLAS single antitop y (normalised)  &     \\
  &  CMS 3D dijets 8 TeV  &     \\
  &  CMS $t\bar{t}$ absolute $|y_t|$  &     \\
  &  CMS $t\bar{t}$ absolute $|y_t|$  &     \\
  &  CMS $\sigma_{tt}^{\rm tot}$ 5 TeV  &     \\
  &  ATLAS DY 2D 8 TeV  &     \\
  &  CMS single top Rt 8 TeV  &     \\
  &  CMS dijets 7 TeV  &     \\
  &  ATLAS $t\bar{t}$ normalised $|y_t|$  &     \\
  &  ATLAS jets 8 TeV, R=0.6  &     \\
  &  ATLAS $W,Z$ inclusive 13 TeV  &     \\
  &  ATLAS single top Rt 13 TeV  &     \\
  &  CMS single top $\sigma(t+\bar{t})$ 7 TeV  &     \\
  &  ATLAS single top $y_t$ (normalised)  &     \\
  &  ATLAS $W^++$jet 8 TeV  &     \\
  &  CMS $t\bar{t}$ double differential $(m_{t\bar{t}}, y_t)$  &     \\
  &  CMS single top $R_t$ 13 TeV  &     \\
  &  ATLAS $W^+-$jet 8 TeV  &     \\
  &  LHCb $Z\to ee$  &     \\
  &  LHCb $Z\to \mu\mu$  &     \\
  &  ATLAS dijets 7 TeV, R=0.6  &     \\
  &  ATLAS $t\bar{t}$ $y_{t\bar{t}}$  &     \\
  &  ATLAS single antitop y (normalised)  &     \\
  &  ATLAS single top $y_t$ (normalised)  &     \\
  &  ATLAS $W,Z$ 7 TeV 2011 Forward selection  &     \\
  \bottomrule
 \end{tabular}
 \vspace{0.3cm}
 \caption{\small The datasets that enter in each of the fits used for future testing, see text
 for details.
 %
 Each dataset is associated to a corresponding family of processes.
 %
 The collider Drell-Yan data are separated into inclusive measurements and
 measurements accompanied by extra radiation.
}
\label{table:table_dataset_variations}	
\end{table}
%-------------------------------------------------------------------------------

